From Formulas to Figures: How Visual Elements Impact User Interactions in Educational Videos

Educational videos have become increasingly relevant in today's learning environments. While prior research in laboratory studies has provided valuable insights, analyzing real-world interaction data can enhance our understanding of authentic user behavior. Previous studies have investigated technical aspects, such as the influence of cuts on pausing behavior, but the impact of visual complexity remains understudied. In this paper, we address this gap and propose a novel approach centered on visual complexity, defined as the number of visually distinguishable and meaningful elements in a video frame, such as mathematical equations, chemical formulas, or graphical representations. Our study introduces a fine-grained taxonomy of visual objects in educational videos, expanding on previous classifications. Applying this taxonomy to 25 videos from physics and chemistry, we examine the relationship between visual complexity and user behavior, including pauses, in-video navigation, and session dropouts. The results indicate that increased visual complexity, especially of textual elements, correlates with more frequent pauses, rewinds, and dropouts. The results offer a deeper understanding of how video design affects user behavior in real-world scenarios. Our work has implications for optimizing educational videos, particularly in STEM fields. We make our code publicly available (https://github.com/TIBHannover/from_formulas_to_figures).

==> algo/dtw.tex <==
\begin{algorithm}[tb]
\caption{Modified Dynamic Time Warping (DTW) Algorithm}
\label{alg:dtw}
\begin{algorithmic}[1] 
    \REQUIRE Two sequences \( s_1 \) and \( s_2 \)
    \REQUIRE \texttt{window}: Size of the warping window
    
    \STATE Initialize distance matrix \( D \) with shape \( (len(s_2), len(s_1)) \)
    
    \FOR{each \( i \) in \( 1 \) to \( len(s_2) \)}
        \FOR{each \( j \) in \( 1 \) to \( len(s_1) \)}
            \STATE \( D[i, j] = (s_1[j] - s_2[i])^2 \)
        \ENDFOR
    \ENDFOR

    \STATE Set distance matrix outside of window to \( \infty \)

    \STATE Initialize cost matrix \( C \) with shape \( (len(s_2), len(s_1)) \)
    \STATE \( C[0, 0] = D[0, 0] \)
    
    \FOR{each \( i \) in [\( 1 \), ..., \( len(s_2) \)]}
        \STATE \( C[i, 0] = D[i, 0] + C[i-1, 0] \)
    \ENDFOR
    
    \FOR{each \( j \) in [\( 1 \), ..., \( len(s_1) \)]}
        \STATE \( C[0, j] = D[0, j] + C[0, j-1] \)
    \ENDFOR
    
    \FOR{each \( i \) in [\( 1 \), ..., \( len(s_2) \)]}
        \FOR{each \( j \) in [\( 1 \), ..., \( len(s_1) \)]}
            \STATE \( C[i, j] = D[i, j] + \min(C[i-1, j], C[i, j-1], C[i-1, j-1]) \)
        \ENDFOR
    \ENDFOR
    
    \STATE Calculate total cost as \( \text{total\_cost} = \frac{C[len(s_2)-1, len(s_1)-1]}{len(path)} \)
    \RETURN \( \text{total\_cost} \), optimal path
\end{algorithmic}
\end{algorithm}

==> algo/dtw_listing.tex <==
\begin{lstlisting}[language=Python, caption={Modified Dynamic Time Warping (DTW) Algorithm}, label={alg:dtw}]
# Require: Two sequences s1 and s2
# Require: window: Size of the warping window

# Initialize distance matrix D
D = np.zeros((len(s2), len(s1)))

for i in range(1, len(s2)):
    for j in range(1, len(s1)):
        D[i, j] = (s1[j] - s2[i]) ** 2

# Set distance matrix outside of window to infinity
D[D > window] = float('inf')

# Initialize cost matrix C
C = np.zeros((len(s2), len(s1)))
C[0, 0] = D[0, 0]

for i in range(1, len(s2)):
    C[i, 0] = D[i, 0] + C[i-1, 0]

for j in range(1, len(s1)):
    C[0, j] = D[0, j] + C[0, j-1]

for i in range(1, len(s2)):
    for j in range(1, len(s1)):
        C[i, j] = D[i, j] + min(C[i-1, j], C[i, j-1], C[i-1, j-1])

# Calculate total cost
total_cost = C[len(s2)-1, len(s1)-1] / len(path)
return total_cost, optimal_path
\end{lstlisting}

==> tables/significance_table_old.tex <==
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{.25cm}
    \caption{Comparison of p-values and permutation effect sizes (PES) for visual complexity (VisCom) and binary visual changes across different user actions and modalities. Significant results are highlighted in bold and underlined.}
    \label{table:significance}
    \begin{tabular}{ccccccc}
    \toprule
    \textbf{} & \textbf{} & \textbf{} & \multicolumn{2}{c}{\textbf{VisCom}} & \multicolumn{2}{c}{\textbf{Binary}} \\
    \textbf{action} & \textbf{modality} & \textbf{time} & \textbf{p-value} & \textbf{PES} & \textbf{p-value} & \textbf{PES} \\
    \midrule
    \multirow{3}{*}{pause} & both & \multirow{6}{*}{/} & {\ul \textbf{0}} & {\ul \textbf{3.15}} & {\ul \textbf{0.012}} & {\ul \textbf{2.08}} \\
     & textual &  & {\ul \textbf{0}} & {\ul \textbf{4.12}} & {\ul \textbf{0.003}} & {\ul \textbf{2.49}} \\
     & visual &  & {\ul \textbf{0.009}} & {\ul \textbf{-2.28}} & 0.068 & -1.49 \\
    \multirow{3}{*}{dropout} & both &  & 0.130 & 1.19 & 0.448 & 0.13 \\
     & textual &  & 0.069 & 1.53 & 0.462 & -0.09 \\
     & visual &  & 0.110 & -1.22 & 0.055 & -1.60 \\
     \midrule
    \multirow{3}{*}{rewind} & both & \multirow{6}{*}{source} & {\ul \textbf{0.002}} & {\ul \textbf{3.03}} & {\ul \textbf{0.002}} & {\ul \textbf{2.90}} \\
     & textual &  & {\ul \textbf{0}} & {\ul \textbf{3.54}} & {\ul \textbf{0.001}} & {\ul \textbf{3.06}} \\
     & visual &  & 0.290 & -0.57 & 0.477 & 0.04 \\
    \multirow{3}{*}{skip} & both &  & 0.181 & -0.92 & 0.029 & -1.90 \\
     & textual &  & 0.056 & -1.63 & {\ul \textbf{0.004}} & {\ul \textbf{-2.54}} \\
     & visual &  & 0.391 & 0.27 & {\ul \textbf{0.004}} & {\ul \textbf{-2.62}} \\
     \midrule
    \multirow{3}{*}{rewind} & both & \multirow{6}{*}{target} & {\ul \textbf{0.012}} & {\ul \textbf{2.29}} & 0.027 & 1.91 \\
     & textual &  & {\ul \textbf{0.019}} & {\ul \textbf{2.22}} & 0.078 & 1.40 \\
     & visual &  & 0.353 & 0.32 & 0.325 & -0.45 \\
    \multirow{3}{*}{skip} & both &  & 0.071 & 1.47 & 0.267 & -0.62 \\
     & textual &  & 0.127 & 1.12 & 0.255 & -0.67 \\
     & visual &  & 0.253 & 0.67 & {\ul \textbf{0.016}} & {\ul \textbf{-2.11}} \\
     \bottomrule
    \end{tabular}
\end{table}
